A Quantitative Study of Security Bug Fixes of GitHub Repositories

Software is prone to bugs and failures. Security bugs are those that expose or share privileged information and access in violation of the software's requirements. Given the seriousness of security bugs, there are centralized mechanisms for supporting and tracking these bugs across multiple products, one such mechanism is the Common Vulnerabilities and Exposures (CVE) ID description. When a bug gets a CVE, it is referenced by its CVE ID. Thus we explore thousands of Free/Libre Open Source Software (FLOSS) projects, on Github, to determine if developers reference or discuss CVEs in their code, commits, and issues. CVEs will often refer to 3rd party software dependencies of a project and thus the bug will not be in the actual product itself. We study how many of these references are intentional CVE references, and how many are relevant bugs within the projects themselves. We investigate how the bugs that reference CVEs are fixed and how long it takes to fix these bugs. The results of our manual classification for 250 bug reports show that 88 (35%), 32 (13%), and 130 (52%) are classified into "Version Update", "Fixing Code", and "Discussion". To understand how long it takes to fix those bugs, we compare two periods, Reporting Period, a period between the disclosure date of vulnerability information in CVE repositories and the creation date of the bug report in a project, and Fixing Period, a period between the creation date of the bug report and the fixing date of the bug report. We find that 44% of bug reports that are classified into "Version Update" or "Fixing Code" have longer Reporting Period than Fixing Period. This suggests that those who submit CVEs should notify affected projects more directly.

==> Makefile <==
FILE_NAME :=report

TEMP_FILES := \
	$(FILE_NAME).aux \
	$(FILE_NAME).bbl \
	$(FILE_NAME).log \
	$(FILE_NAME).blg \
	$(FILE_NAME).brf \
	$(FILE_NAME).dvi \
	$(FILE_NAME).out

SECTION_FILES = \
	$(FILE_NAME).tex \
	intro.tex \
	reference.tex \
	dataset.tex \
	RQ1.tex \
	RQ2.tex \
	RQ3.tex \
	validity.tex \
	conclusion.tex

BIBTEX_FILES = BugFix.bib

GEN_FIGURES = \

STATIC_FIGURES = #./img/* \

TABLES = #./table/* \

DEBUG=yes
ifneq '$(DEBUG)' 'yes'
LATEX_FLAGS="-interaction=batchmode --file-line-error --synctex=1"
endif
LATEX_FLAG_ENC="-kanji=utf8"
OPEN ?= open

.DELETE_ON_ERROR:

################################################################################
# Main paper building
################################################################################


$(FILE_NAME).pdf: $(SECTION_FILES) $(GEN_FIGURES) $(STATIC_FIGURES) $(TABLES) $(BIBTEX_FILES)
	platex $(LATEX_FLAGS) $(FILE_NAME)
	pbibtex $(FILE_NAME)
	platex $(LATEX_FLAGS) $(FILE_NAME)
	platex $(LATEX_FLAGS) $(FILE_NAME)
	dvipdfmx $(FILE_NAME)

.PHONY: clean view
clean:
	rm -f $(TEMP_FILES) $(GEN_FIGURES) $(FILE_NAME).pdf

view: $(FILE_NAME).pdf
	$(OPEN) $(FILE_NAME).pdf

